Beyond Prediction: Tail-Aware Scheduling for LLM Inference

LLM serving exhibits extreme length variability, making size-based scheduling difficult in practice. Recent LLM schedulers approximate SJF/SRPT using predicted decode lengths or ranks and primarily report mean-centric metrics such as TTFT and TBT. We show that these prediction-driven policies can be fragile under distribution shifts, bursty arrivals, and GPU memory pressure, while offering limited control over the tail latency (P90-P99) that dominates user experience, even with perfect decode-length knowledge. We introduce a distribution-aware, prediction-free scheduling framework that replaces explicit length prediction with soft priority boosting driven by lightweight statistical signals. Our design co-optimizes scheduling and cache-aware preemption to account for memory-coupled decode dynamics across workload mixes. Evaluated on production and open-source traces, our method reduces P99 TTLT by up to 35-50% relative to SRPT with perfect length knowledge and reduces TTFT by 34-47% across workloads, including reasoning-heavy and chat-heavy tasks. These results demonstrate a robust alternative for optimizing tail latency in online LLM serving.

==> Sections/07-Related-Work.tex <==

\section{Related Work}
\input{Sections/table/comparison_related}
\paragraph{Size-Based Scheduling for LLM Serving.}

Motivated by classical results that SJF/SRPT minimize mean response time when job sizes are known, recent LLM serving systems adopt size-based prioritization using predicted output length. Fu et al. propose a learning-to-rank (LTR) scheduler that approximates SJF by predicting generation lengths, demonstrating improvements in mean and P90 TTFT and time-between-token latencies~\cite{fu2024efficient}. Related approaches such as TRAIL (embedding-based schedulers) similarly rely on learned predictors to estimate remaining execution tokens and guide preemptive scheduling decisions, with a threshold to help reduce preemption at a later phase~\cite{shahout2024don}. Heuristic methods in SGLang and vLLM, such as Shortest Prefix First (SPF), avoid explicit output prediction by using the known prefill length as a proxy for the total job size, thereby ignoring the high variance in decoding length that can impact throughput and TTLT. 



\paragraph{Metric Mismatch: Mean vs. Tail-Optimality in LLM Serving.  }

% In LLM application and serving systems, user experience is often dominated by tail latency~\cite{Shinjuku,zhang2025tail,li2024libpreemptible,yu2022orca,zhong2024distserve,patel2023splitwise}. \yueying{This may sound a bit aggresive to put in the front, but they do omit P90/P95/P99 latencies} Tail metrics (e.g., P95/P99 TTFT/TTLT) are largely absent from the evaluation of prediction-based SJF/SRPT schedulers \cite{fu2024efficient,shahout2024don}. FastServe~\cite{wu2023fast} adopts a skip-join multi-level feedback queue (MLFQ), without the need of knowing job sizes, assigning request priorities based on the length generated so far. While MLFQ can trade off fairness and latency, maintaining multiple priority queues adds complexity for batching and interactive LLM workloads. Furthermor, it is only mean optimal for heavy-tailed job size distribution. In LLM, response lengths are often capped, and some applications are more light-tailed, which makes SJF/SRPT/MLFQ arbitrarily bad in tail theoretically~(such as s1k distribution in Fig~\ref{fig:distribution-s1k}).  
LLM serving is typically \emph{SLO-constrained}: the sustainable load of a serving stack is set by whether it can keep \emph{tail} latencies within budget under burstiness and heterogeneous request lengths~\cite{Shinjuku,yu2022orca,zhong2024distserve,zhang2025tail,li2024libpreemptible,patel2023splitwise,goel2025niyama}.
Accordingly, \textbf{tail completion time}---\emph{Time-To-Last-Token} (TTLT) at P95/P99---directly captures user-perceived responsiveness for end-to-end tasks and often becomes the binding constraint in practice.
In contrast, focusing on \emph{mean} TTFT/TBT can be misleading.
First, token-level means do not compose: small per-token slowdowns can accumulate over long generations, yielding acceptable mean TTFT/TBT but poor P95/P99 TTLT.
Second, mean metrics can mask \emph{distributional pathologies}: policies that improve the average by favoring short (or partially served) requests may still create stragglers via starvation or head-of-line effects, inflating tail TTLT even when mean TTFT appears benign.

Despite this, tail metrics (e.g., P95/P99 TTFT/TTLT) are often under-reported in evaluations of size- or prediction-driven schedulers~\cite{fu2024efficient,shahout2024don}.
More fundamentally, mean-optimality does not imply tail-robustness: when response lengths are capped and some traces become closer to light-tailed (e.g., Fig.~\ref{fig:distribution-s1k}), size-based prioritization can be \emph{arbitrarily bad}. In fact, PS and SRPT can achieve the worst possible sojourn-time decay rate (same as PLCFS) under mild condition~\cite{nair2010scheduling}. 


%R Moreover, aggressive size-based preemption—especially when driven by noisy predictions—can reduce mean TTFT while worsening tail latency or inducing jittery token streams, effects that are not reflected in mean-centric metrics. While effective for reducing average latency, these approaches are fundamentally aligned with mean-optimal scheduling objectives. Consequently, prior evaluations predominantly focus on mean TTLT or mean TTFT—metrics for which SJF/SRPT-style policies are theoretically optimal—but provide limited insight into tail behavior, which is often the binding constraint in production SLOs. \emph{Furthermore, we observe that the }



\paragraph{Practical Constraints: Fairness and Memory-Coupled Preemption.}

Another challenge for SRPT-style scheduling in LLM serving arises from KV-cache-coupled execution and fairness. First, SJF/SRPT may lead to starvation for long-running requests. Unlike previous fairness-promoting design~\cite{sheng2024fairness}, which focuses on fairness between different clients, LTR proposes a \maxtpot fairness metric to evaluate fairness at the per-request level to prevent starvation due to SJF~\cite{fu2024efficient}. 
One limitation is that \maxtpot is dominated by a single worst inter-token stall: transient batching/memory events can inflate \maxtpot and trigger quantum promotions even when a request is not persistently starved, which may destabilize batching/KV locality and reduce overall throughput under load. \yueying{This seems like detail I can move later}


 During decoding, requests accumulate large key–value (KV) caches that must be preserved across preemption, making late-stage interruption costly. Systems such as Sarathi-Serve and PagedAttention focus on improving throughput–latency tradeoffs and memory efficiency, but do not directly address tail-optimal scheduling under preemption overheads \cite{agrawal2024taming,kwon2023efficient}. While some prediction-based schedulers introduce heuristics to limit preemption, they do not fundamentally mitigate the brittleness of prediction-driven priority inversion under workload variability.

\paragraph{Tail-optimal Scheduling in Queuing Theory.}
A rich body of queueing-theoretic work studies scheduling policies that optimize tail behavior of response times. For systems with heavy-tailed job sizes, policies such as LAS and variants of age-based scheduling are known to achieve favorable tail properties without requiring job size information \cite{scully2020characterizing}. More recently, Harlev et al. develop a Gittins-index policy that explicitly targets tail latency optimization under stochastic service dynamics \cite{harlev2025gittins}. Complementary to these results, Yu and Scully establish strong tail optimality for the $\gamma$-Boost policy in light-tailed M/G/1 queues, showing that soft, continuous boosting improves not only the exponential decay rate but also the tail constant of response time distributions \cite{yu2024strongly}. These works highlight a fundamental distinction between mean optimality and tail optimality, motivating scheduling designs that go beyond average latency.

\paragraph{This Work: Bridging Queuing with LLM System Optimization.}

Unlike prior LLM schedulers based on SJF or SRPT (e.g. LTR and TRAIL~\cite{shahout2024don,fu2024efficient}), which primarily optimize
mean end-to-end latency or mean TTFT and rely on decoding-size or length rank prediction, our approach explicitly targets
tail-latency metrics, including high-percentile TTFT and TTLT. 
\textbf{\emph{This distinction is fundamental: while SJF/SRPT are mean-optimal, they offer no guarantees on tail behavior, especially under bursty loads, diverse request input/output length distribution and continuous batching (outside of M/G/1 assumption) with memory constraints. } } Table~\ref{tab:scheduler-comparison} shows the key distinctions in our work w.r.t workload distribution (heavy-tailed, light-tailed), key assumptions (no size prediction) and the design (preemption-aware, tail-aware, TLLT-aware). 


